Causal Unsupervised Semantic Segmentation

Unsupervised semantic segmentation aims to achieve high-quality semantic grouping without human-labeled annotations. With the advent of self-supervised pre-training, various frameworks utilize the pre-trained features to train prediction heads for unsupervised dense prediction. However, a significant challenge in this unsupervised setup is determining the appropriate level of clustering required for segmenting concepts. To address it, we propose a novel framework, CAusal Unsupervised Semantic sEgmentation (CAUSE), which leverages insights from causal inference. Specifically, we bridge intervention-oriented approach (i.e., frontdoor adjustment) to define suitable two-step tasks for unsupervised prediction. The first step involves constructing a concept clusterbook as a mediator, which represents possible concept prototypes at different levels of granularity in a discretized form. Then, the mediator establishes an explicit link to the subsequent concept-wise self-supervised learning for pixel-level grouping. Through extensive experiments and analyses on various datasets, we corroborate the effectiveness of CAUSE and achieve state-of-the-art performance in unsupervised semantic segmentation.

==> old_writing.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 더 옛날 overview
% We begin with explaining why to use frontdoor adjustment for unsupervised semantic segmentation (USS). To successfully perform it, we first explain how to create a mediator (\textit{i.e.,} a concept cluster book), by utilizing the idea of \textit{Modularity}~\citep{newman2006modularity} in graph theory. It can measure the structure of features within a graph, capturing the strength of division into groups, clusters, or communities. Here, the mediator plays a role in collecting discretized candidate features of final clusters according to dataset, possibly representing rich features in pre-trained model. Second, by using this mediator, we learn to enhance likelihood of segmentation outcome with all possible treatments (\textit{i.e.,} in-batch and out-batch features), which have a strong effect in searching similar features and learning to resemble themselves in total datasets. With the two steps, we present a framework of causal unsupervised semantic segmentation (CUSS) addressing the chronic issue of ``what to cluster''. Furthermore, we present transformer-based segmentation head inspired by \citet{vaswani2017attention, carion2020end} to more focus on concept-attended features, which is followed by MLP-based segmentation head used in STEGO~\citep{hamilton2022unsupervised} and HP~\citep{seong2023leveraging}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 더 옛날 overview
% \paragraph{Overview.} We start with defining the unsupervised tasks for segmentation and exploring how they can be bridged to causal inference, particularly through frontdoor adjustment. Overall training procedure of our framework is illustrated in Fig.~\ref{fig:3}. As in the figure, we first introduce the construction process of a mediator (\textit{i.e.,} concept \textit{clusterbook}), by utilizing the idea of \textit{Modularity}~\citep{newman2006modularity} in discretized manners. Second, by using the indices in the clusterbook, we train a prediction head to enhance likelihood of segmentation outcome considering all possible treatments (\textit{i.e.,} in-batch and out-batch features) through self-supervised learning. In the following sections, we delve into each task in detail.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 기존의 overview
\paragraph{Overview.} We start with defining the unsupervised tasks for USS and exploring how they can be bridged to causal inference, particularly through frontdoor adjustment. Overall training procedure of our framework is illustrated in Fig.~\ref{fig:3}. As in the figure, we first introduce step 1 task, which involves constructing a mediator (\textit{i.e.,} concept \textit{clusterbook}), by utilizing the idea of \textit{Modularity}~\citep{newman2006modularity}. It can measure the structure of features within a graph, capturing the strength of division into groups, clusters, or communities. Here, constructing the mediator indicates a task of discretizing as many subdivided concept candidates from the pre-trained feature representation as possible. These discretized prototypes play a crucial role in assigning categorized indices to concept fractions, providing explicit guidance for subsequent semantic grouping. Secondly, in step 2, we use the clusterbook to train a segmentation head and enhance the likelihood of segmentation outcomes, considering all possible treatments (\textit{i.e.,} in-batch and out-batch features) through self-supervised learning. This strategy strongly influences the search for similar features and consolidates semantic concepts into the broader-level categories we target. After explaining the data generating process of USS in a causal perspective, we delve into each task in detail in the following sections.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 가장 최근 overview
%We start with defining the unsupervised tasks for USS and exploring how they can be bridged to causal inference, particularly through frontdoor adjustment. Overall training procedure of our framework is illustrated in Fig.~\ref{fig:3}. As in the figure, we first extract subdivdied concept fractions in step 1 (\textit{e.g.,} head, torso, hands, legs, sky, water, ball, etc) from pre-trained features by utilizing the idea of \textit{Modularity}~\citep{newman2006modularity}. In step 2, we compute the concept distance between concept fractions and cluster features with closer distances (\textit{e.g.,} head, torso, hands, legs) and separate them with the far distance (\textit{e.g.,} sky, water, ball), thereby enabling to get broader-level category (\textit{e.g.,} human, sky, water, ball).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Similarly, the task of USS has a challenging problem as it is difficult to define what to cluster and how to do so with different level of granularity depending on objects (\textit{e.g.,} head, torso, hand, leg, etc.) shown in Fig.~\ref{fig:1}, considered as confounder $U$, due to the absence of human-biased annotations in dataset.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In detail, a measure of modularity $\mathcal{Q}$ can be written as $1/2e \sum_{i,j}[\mathcal{A}_{ij}-d_id_j/2e]\delta(i.j)$ where $\mathcal{A}\in\mathbb{R}^{hw\times hw}$ indicates the affinity matrix of $T\in\mathbb{R}^{hw\times c}$ representing how much the connectivity exists in vertices such that $\mathcal{A}_{ij}=\exp(-\text{dist}(t_i, t_j))$ if $i\neq j$ and $\mathcal{A}_{ij}=0$ if $i=j$. Note that, $t_i, t_j\in T$ represents the two feature points having $\mathbb{R}^{c}$ dimension. Degree vector $d\in\mathbb{R}^{hw}$ describes the number of the connectivity edges corresponding to its affinity $\mathcal{A}$, and $e\in\mathbb{R}$ denotes the total number of the edges. In addition, $\delta(i, j)$ represents the discriminator of same group where it is one if the two feature points $t_{i}$ and $t_{j}$ are equal group and zero if it is not. Here, the measure of modularity $\mathcal{Q}$ having theoretical range from $-1$ to $1$ displays how features are well separated and clustered: good cluster if it is close to one, otherwise on the contrary.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
However, it is widely acknowledged that maximizing modularity is a practically intractable task due to its NP-hard nature~\citep{brandes2006maximizing}, arising from the challenge of identifying all possible combinations $\delta(i, j)$. To address this issue, \citet{newman2004finding} propose a spectral relaxation approach, which can be expressed as follows:
\begin{equation}
    \hat{\mathcal{Q}} = \frac{1}{2e}\text{Tr}\left(\mathcal{C}^T\left[\mathcal{A}-\frac{dd^T}{2e}\right]\mathcal{C}\right)\in\mathbb{R},
\label{eqn:modularity}
\end{equation}
where $\mathcal{C}\in\mathbb{R}^{hw\times k}$ denotes cluster assignment matrix representing which cluster features are assigned to, such that $k$ describes the concept number of clusterbook $M\in\mathbb{R}^{k\times c}$. To adapt it to USS, we treat $\mathcal{C}$ as a soft assignment matrix and compute it using cosine similarity between rich features $T$ and concept clusters $M$ such that $\mathcal{C}=\max(0, \text{cos}(T, M))\in\mathbb{R}^{hw\times k}$ where they are all normalized when computing cosine similarity. In addition, affinity matrix is also computed with it such that $\mathcal{A}_{ij}=\max(0, \text{cos}(t_i, t_j))$ if $i\neq j$ and $\mathcal{A}_{ij}=0$ if $i=j$ between the two feature points $t_i, t_j\in\mathbb{R}^{c}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Here, we consider $\hat{\mathcal{Q}}$ as $\mathbb{E}_t[\mathbb{E}_m[p(m|t)]]\in\mathcal{R}$ such that $m\in\mathbb{R}^{c}$ denotes a concept in $M$. Next, we maximize it to effectively compress rich information of $T$ while preserving the locality (\textit{i.e,} different level of granularity) around the features, such that $\max_{M}\hat{\mathcal{Q}}=\mathbb{E}_t[\mathbb{E}_m[p(m|t)]]$. Note that, we assume $\hat{\mathcal{Q}}$ has a positive value since pre-trained model representation $T$ has been already clustered well through self-supervised learning~\citep{caron2021emerging, oquab2023dinov2, he2022masked}. In practical, directly calculating Eq.~(\ref{eqn:modularity}) can lead to much small value of $\hat{\mathcal{Q}}$ due to multiplying tiny elements of $\mathcal{C}$ twice. To overcome this, we use trace property and hyperbolic tangent with temperature term $\tau$ to scale up $\mathcal{C}$, while maintaining the maximum of two multiplication for cosine similarity to one. Algorithm~\ref{alg:mediator} provides more details on achieving maximizing modularity to generate concept clusterbook $M$, where we train one epoch by using AdamW~\citep{loshchilov2018decoupled}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BK v2
%For the given patch feature $t\in\mathbb{R}^{c}$ as an anchor, we can find the most similar concept $q\in\mathbb{R}^{c}$ (\textit{e.g.,} head) and its index: $\text{id}_{q}$ such that $q=\arg\max_{m\in M} \mathcal{C}(m, t)$. Then, $\mathcal{D}_{M}[\text{id}_{q}, :]\in\mathbb{R}^{k}$ in pseudo-code-like manner represents concept-wise distances between the most similar concept $q\in\mathbb{R}^{c}$ for the given $t$ and all concept prototypes in $M\in\mathbb{R}^{k\times c}$. Here, we opt for soft relaxation when selecting positive concepts $m^{+}$, because the main purpose in our unsupervised setup is to group subdivided concept prototypes into desired broader-level categories where the relaxed clustering is already fulfilled on the effects of soft positive mining. Therefore, we set positive relaxation $\phi^{+}$ to softly $0.3$ in order to discriminate which concepts are similar with $q$ in terms of broad-level categories, so that we gather positive concepts $m^{+}$ (\textit{e.g.,} torso, hand, leg, etc) from $q$ (\textit{e.g.,} head) satisfying $\mathcal{D}_M[\text{id}_{q}, :]>\phi^{+}$. On the other hand, we set negative relaxation $\phi^{-}$ to hard $0.1$ for stockpiling negative concepts $m^{-}$ (\textit{e.g.,} sky, water, ball, etc) from $q$ (\textit{e.g.,} head) satisfying $\mathcal{D}_M[\text{id}_{q}, :]<\phi^{-}$, since hard negative mining is crucial to perform self-supervised learning~\citep{jaiswal2020survey, khosla2020supervised, kalantidis2020hard, robinson2021contrastive, wang2021exploring}. Note that, there is a few case that the row vector in $\mathcal{D}_M$ has a minimum value over $0$, thus we technically set hard negative relaxation to $0.1$ instead of $0$. Next, we first sample in-batch positive and negative features by using prototype embedding $Q=\{q\in\mathbb{R}^{c}\}^{hw}$ where a positive patch feature point $t^{+}$ is collected if the corresponding $q$ is included in $m^{+}$ and a negative patch feature point $t^{-}$ is collected if $q$ is included in $m^{-}$. Among $Y=\{y\in\mathbb{R}^{r}\}^{hw}$ get from segmentation head $S$, the feature points $y$ spatially corresponding to $t^{+}$ and $t^{-}$ are selected to be positive and negative features $y^{+}$ and $y^{-}$. From this selection, we aim to compute the concept distance between concept prototypes and cluster features $Y$ with closer distance concepts (\textit{e.g.,} head, torso, hands, legs) and separate them with the far distance concepts (\textit{e.g.,} sky, water, ball), thereby enabling to get broader-level categories (\textit{e.g.,} human, sky, water, ball).
%%%%%%%%%%%%%%%%%%%%%%


%Later, all of the stocked positive and negative feature points are propagated through segmentation head $S$, resulting as $y^{+}$ and $y^{-}$.
%for self-supervised learning using Eq.~(\ref{eqn:likelihood_modification}).

%From this, we heuristically set positive relaxation $\phi^{+}$ to softly $0.3$ in order to discriminate which concepts are similar with $m$ through retrieval visualization results described in Appendix~\label{appendix:}, so that we gather positive concepts $m^{+}$ only satisfying $\mathcal{D}_M[\text{id}_{m}]>\phi^{+}$ and then collect all of the positive feature points $t'^{+}$ corresponding to $m^{+}$. On the other hand, we initially set negative relaxation $\phi^{-}$ to $0$ for stockpiling negative concepts $m^{-}$ satisfying $\mathcal{D}_M[\text{id}_{m^{*}}]<\phi^{-}$ and assembling all of the negative feature points $t'^{-}$ corresponding to $m^{-}$. This is because mining hard negative samples is crucial to progress self-supervise learning based on numerous consistent studies~\citep{jaiswal2020survey, khosla2020supervised, kalantidis2020hard, robinson2021contrastive, wang2021exploring}. However, there are a few case that the row vector in $\mathcal{D}_M$ has a minimum value over zero, thus we technically set hard negative relaxation to $0.1$. Later, all of the stocked positive and negative feature points $t'^{+}$ and $t'^{-}$ are propagated through segmentation head $S$ and then the propagated ones are each heaped in a shape of $y^{+}$ and $y^{-}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
